Diffusion-Based 3D Human Pose Estimation with Multi-Hypothesis Aggregation

In this paper, a novel Diffusion-based 3D Pose estimation (D3DP) method with Joint-wise reProjection-based Multi-hypothesis Aggregation (JPMA) is proposed for probabilistic 3D human pose estimation. On the one hand, D3DP generates multiple possible 3D pose hypotheses for a single 2D observation. It gradually diffuses the ground truth 3D poses to a random distribution, and learns a denoiser conditioned on 2D keypoints to recover the uncontaminated 3D poses. The proposed D3DP is compatible with existing 3D pose estimators and supports users to balance efficiency and accuracy during inference through two customizable parameters. On the other hand, JPMA is proposed to assemble multiple hypotheses generated by D3DP into a single 3D pose for practical use. It reprojects 3D pose hypotheses to the 2D camera plane, selects the best hypothesis joint-by-joint based on the reprojection errors, and combines the selected joints into the final pose. The proposed JPMA conducts aggregation at the joint level and makes use of the 2D prior information, both of which have been overlooked by previous approaches. Extensive experiments on Human3.6M and MPI-INF-3DHP datasets show that our method outperforms the state-of-the-art deterministic and probabilistic approaches by 1.5% and 8.9%, respectively. Code is available at https://github.com/paTRICK-swk/D3DP.

==> table/3dhp.tex <==
\begin{center}
  %\centering
  %\renewcommand\tabcolsep{4.0pt}
%\vspace{-0.1cm}
%\vspace{-0.4cm}
\renewcommand{\arraystretch}{0.7}
\resizebox{\linewidth}{!}{\begin{tabular}{c|ccc}
\hline\noalign{\smallskip}
Method&PCK$\uparrow$&AUC$\uparrow$&MPJPE$\downarrow$\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
U-CDGCN~\cite{hu2021conditional} ACMMM'21 ($N$=96)$\triangledown$&97.9&69.5&42.5\\
P-STMO~\cite{shan2022p} ECCV'22 ($N$=81)$\triangledown$ &97.9&75.8&32.2\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
% Mehta \textit{et al.}~\cite{mehta2017monocular} 3DV'17 ($N$=1)&75.7&39.3&117.6\\
TCN~\cite{pavllo20193d} CVPR'19 ($N$=81)&86.0&51.9&84.0\\
% Lin \textit{et al.}~\cite{lin2019trajectory} BMVC'19 ($N$=25)&83.6&51.4&79.8\\
% Zeng \textit{et al.}~\cite{zeng2020srnet} ECCV'20 ($N$=1)&77.6&43.8&-\\
U-GCN~\cite{wang2020motion} ECCV'20 ($N$=96)&86.9&62.1&68.1\\
Anatomy~\cite{chen2021anatomy} TCSVT'21 ($N$=81)&87.9&54.0&78.8\\
PoseFormer~\cite{zheng20213d} ICCV'21 ($N$=9)&88.6&56.4&77.1\\
MHFormer~\cite{li2022mhformer} CVPR'22 ($N$=9, $H$=3, P-Agg)&93.8&63.3&58.0\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=27)&94.4&66.5&54.9\\


MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)$\ddagger$&\textcolor{blue}{96.9}&75.8&35.4\\
\bestcell{D3DP ($N$=243, $H$=1, $K$=1)}&\bestcell{\textcolor{red}{97.7}}&\bestcell{77.8}&\bestcell{30.2}\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=20, P-Agg)}&\bestcell{\textcolor{red}{97.7}}&\bestcell{\textcolor{blue}{78.0}}&\bestcell{\textcolor{blue}{30.0}}\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=20, J-Agg)}&\bestcell{\textcolor{red}{97.7}}&\bestcell{\textcolor{red}{78.2}}&\bestcell{\textcolor{red}{29.7}}\\

\noalign{\smallskip}
\hline
\noalign{\smallskip}

\bestcell{D3DP ($N$=243, $H$=20, $K$=20, P-Best$\sharp$)}&\bestcell{\textcolor{blue}{97.8}}&\bestcell{\textcolor{blue}{78.2}}&\bestcell{\textcolor{blue}{29.8}}\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=20, J-Best$\sharp$)}&\bestcell{\textcolor{red}{98.0}}&\bestcell{\textcolor{red}{79.1}}&\bestcell{\textcolor{red}{28.1}}\\
\noalign{\smallskip}
\hline
\end{tabular}}
\end{center}
%\vspace{-0.6cm}

==> table/ablation.tex <==
\newcommand\tr{\rule{0pt}{10pt}}
\newcommand\br{\rule[-3.3pt]{0pt}{3.3pt}}
%#################################################
% Component
%#################################################
\subfloat[
Component. J-Agg: use JPMA.
\label{tab:component}
]{
\centering
\begin{minipage}{0.23\linewidth}{\begin{center}
\tablestyle{2pt}{1.05}
%\begin{tabular}{x{20}x{20}x{10}x{25}x{30}}
\begin{tabular}{ccccc}
\shline
D3DP & JPMA & $H$ & Setting &MPJPE$\downarrow$ \\
\shline
&&  1 &N/A&41.0 \\
\checkmark && 1&N/A&40.0 \\
\checkmark && 20&P-Agg&39.9 \\
\bestcell{\checkmark} &\bestcell{\checkmark}&\bestcell{20}&\bestcell{J-Agg}& \bestcell{39.5} \\
\shline
\end{tabular}
\end{center}}
\end{minipage}
}
\hspace{0.01\linewidth}
%#################################################
% Multi-hypothesis aggregation
%#################################################
\subfloat[
Hypothesis aggregation. $H$=20
\label{tab:MHA}
]{
\begin{minipage}{0.22\linewidth}{
\begin{center}
\tablestyle{1.3pt}{1.05}
\begin{tabular}{x{28}x{40}x{30}}
%\begin{tabular}{ccc}
\shline
Level & Method &MPJPE$\downarrow$ \\
\shline
pose & average &39.9 \\
pose & MLPs &42.5 \\
joint & MLPs &41.6 \\
\bestcell{joint}& \bestcell{JPMA} & \bestcell{39.5}\\
joint & JPMA-var. &39.5 \\
\shline
\end{tabular}
\end{center}
}
\end{minipage}
}
\hspace{0.01\linewidth}
%#################################################
% speed 
%#################################################
\subfloat[
Accuracy\&speed. Setting: J-Agg. MACs is averaged over each frame. 
\label{tab:speed}
]{
\begin{minipage}{0.48\linewidth}{\begin{center}
\tablestyle{1.5pt}{1.05}
%\begin{tabular}{m{20pt}m{10pt}m{10pt}m{30pt}m{30pt}m{45pt}m{45pt}m{25pt}}
\begin{tabular}{>{\centering\arraybackslash}m{20pt}>{\centering\arraybackslash}m{10pt}>{\centering\arraybackslash}m{10pt}>{\centering\arraybackslash}m{30pt}>{\centering\arraybackslash}m{35pt}>{\centering\arraybackslash}m{42pt}>{\centering\arraybackslash}m{42pt}>{\centering\arraybackslash}m{25pt}}

%\begin{tabular}{cccccccc}
\shline
%\br{\# boxes}\tr & step & AP & AP$_{50}$ & AP$_{75}$ & FPS \\
D3DP & $H$ & $K$ &MPJPE$\downarrow$ & Params(M)& Train. MACs(G)&Infer. MACs(G) & Infer. FPS \\
\shline
&1&1&41.0&33.6&0.57&1.14&4547 \\
\checkmark&1&1&40.0&34.6&0.57&1.14&4364 \\
\checkmark&5&1&39.9&34.6&0.57&5.70&886 \\
\checkmark&1&5&40.0&34.6&0.57&5.70&1018 \\
\checkmark&5&5&39.7&34.6&0.57&28.5&204 \\
\bestcell{\checkmark}&\bestcell{20}&\bestcell{10}&\bestcell{39.5}&\bestcell{34.6}&\bestcell{0.57}&\bestcell{228.2}&\bestcell{29} \\

\shline
\end{tabular}
\end{center}}
\end{minipage}
}




==> table/h36m.tex <==
\begin{center}
  %\centering
  %\renewcommand\tabcolsep{4.0pt}
%\vspace{-0.5cm}
\renewcommand{\arraystretch}{0.7}
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccccccccccccccc|c}
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Deterministic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
TCN~\cite{pavllo20193d} CVPR'19 ($N$=243)*& 45.2&46.7&43.3&45.6&48.1&55.1&44.6&44.3&57.3&65.8&47.1&44.0&49.0&32.8&33.9&46.8 \\
% Lin \textit{et al.}~\cite{lin2019trajectory} BMVC'19 ($N$=50)& 42.5&44.8&42.6&44.2&48.5&57.1&42.6&41.4&56.5&64.5&47.4&43.0&48.1&33.0&35.1&46.6 \\
% Xu \textit{et al.}~\cite{xu2020deep} CVPR'20 ($N$=9)
% &\textbf{37.4}&43.5&42.7&42.7&46.6&59.7&41.3&45.1&\textbf{52.7}&60.2&45.8&43.1&47.7&33.7&37.1&45.6\\
% Wang \textit{et al.}~\cite{wang2020motion} ECCV'20 ($N$=96)
% &41.3&43.9&44.0&42.2&48.0&57.1&42.2&43.2&57.3&61.3&47.0&43.5&47.0&32.6&31.8&45.6\\
% Attn-TCN~\cite{liu2020attention} CVPR'20 ($N$=243)& 41.8&44.8&41.1&44.9&47.4&54.1&43.4&42.2&56.2&63.6&45.3&43.5&45.3&31.3&32.2&45.1 \\
SRNet~\cite{zeng2020srnet} ECCV'20 ($N$=243)*& 46.6&47.1&43.9&41.6&45.8&49.6&46.5&40.0&53.4&61.1&46.1&42.6&43.1&31.5&32.6&44.8 \\
% Zeng \textit{et al.}~\cite{zeng2021learning} ICCV'21 ($N$=9)
% &-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&45.7\\
PoseFormer~\cite{zheng20213d} ICCV'21 ($N$=81)*&
41.5&44.8&39.8&42.5&46.5&51.6&42.1&42.0&53.3&60.7&45.5&43.3&46.1&31.8&32.2&44.3\\
RIE~\cite{shan2021improving} ACMMM'21 ($N$=243)*&
40.8&44.5&41.4&42.7&46.3&55.6&41.8&41.9&53.7&60.8&45.0&41.5&44.8&30.8&31.9&44.3\\
Anatomy~\cite{chen2021anatomy} TCSVT'21 ($N$=243)*&
41.4&43.5&40.1&42.9&46.6&51.9&41.7&42.3&53.9&60.2&45.4&41.7&46.0&31.5&32.7&44.1\\
U-CDGCN~\cite{hu2021conditional} ACMMM'21 ($N$=96)*&
38.0&43.3&39.1&\textcolor{blue}{39.4}&45.8&53.6&41.4&41.4&55.5&61.9&44.6&41.9&44.5&31.6&29.4&43.4\\
Ray3D~\cite{zhan2022ray3d} CVPR'22 ($N=9$)*&
44.7&48.7&48.7&48.4&51.0&59.9&46.8&46.9&58.7&61.7&50.2&46.4&51.5&38.6&41.8&49.7\\
STE~\cite{li2022exploiting} TMM'22 ($N$=351)*&
39.9&43.4&40.0&40.9&46.4&50.6&42.1&\textcolor{blue}{39.8}&55.8&61.6&44.9&43.3&44.9&29.9&30.3&43.6\\
P-STMO~\cite{shan2022p} ECCV'22 ($N$=243)*&
38.9&42.7&40.4&41.1&45.6&49.7&40.9&39.9&55.5&59.4&44.9&42.2&42.7&29.4&29.4&42.8\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)*$\ddagger$&
37.9&\textcolor{blue}{40.1}&37.5&\textcolor{blue}{39.4}&43.3&50.0&\textcolor{blue}{39.8}&39.9&52.5&56.6&42.4&40.1&40.5&\textcolor{blue}{27.6}&\textcolor{blue}{27.7}&41.0\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)*&
\textcolor{red}{37.6}&40.9&37.3&39.7&42.3&49.9&40.1&\textcolor{blue}{39.8}&51.7&55.0&42.1&\textcolor{blue}{39.8}&41.0&27.9&27.9&40.9\\
DUE~\cite{zhang2022uncertainty} ACMMM'22 ($N$=300)*&
37.9&41.9&\textcolor{blue}{36.8}&39.5&\textcolor{red}{40.8}&\textcolor{blue}{49.2}&40.1&40.7&\textcolor{red}{47.9}&\textcolor{red}{53.3}&\textcolor{red}{40.2}&41.1&\textcolor{blue}{40.3}&30.8&28.6&\textcolor{blue}{40.6}\\
\bestcell{D3DP ($N$=243, $H$=1, $K$=1)*}&
\bestcell{\textcolor{blue}{37.7}}&\bestcell{\textcolor{red}{39.9}}&\bestcell{\textcolor{red}{35.7}}&\bestcell{\textcolor{red}{38.2}}&\bestcell{\textcolor{blue}{41.9}}&\bestcell{\textcolor{red}{48.8}}&\bestcell{\textcolor{red}{39.5}}&\bestcell{\textcolor{red}{38.3}}&\bestcell{\textcolor{blue}{50.5}}&\bestcell{\textcolor{blue}{53.9}}&\bestcell{\textcolor{blue}{41.6}}&\bestcell{\textcolor{red}{39.4}}&\bestcell{\textcolor{red}{39.8}}&\bestcell{\textcolor{red}{27.4}}&\bestcell{\textcolor{red}{27.5}}&\bestcell{\textcolor{red}{40.0}}\\

\noalign{\smallskip}
\hline
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Probabilistic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Agg)&
48.6&54.5&54.2&55.7&62.6&72.0&50.5&54.3&70.0&78.3&58.1&55.4&61.4&45.2&49.7&58.0\\
GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Agg)&
67.9&75.5&71.8&81.8&81.4&93.7&75.2&81.3&88.8&114.1&75.9&79.1&83.3&74.3&79.0&81.1\\
GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=5, P-Agg)&
51.9&56.1&55.3&58.0&63.5&75.1&53.3&56.5&69.4&92.7&60.1&58.0&65.5&49.8&53.6&61.3\\
NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=1, P-Agg)&
52.4&60.2&57.8&57.4&65.7&74.1&56.2&59.1&69.3&78.0&61.2&63.7&67.0&50.0&54.9&61.8\\
MHFormer~\cite{li2022mhformer} CVPR'22 ($N$=351, $H$=3, P-Agg)*&
39.2&43.1&40.1&40.9&44.9&51.2&40.6&41.3&53.5&60.3&43.7&41.1&43.8&29.8&30.6&43.0
\\
\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Agg)*}&
\bestcell{37.7}&\bestcell{39.9}&\bestcell{\textcolor{blue}{35.7}}&\bestcell{38.2}&\bestcell{41.9}&\bestcell{48.8}&\bestcell{39.5}&\bestcell{38.3}&\bestcell{50.5}&\bestcell{53.9}&\bestcell{41.6}&\bestcell{\textcolor{blue}{39.4}}&\bestcell{39.8}&\bestcell{\textcolor{blue}{27.4}}&\bestcell{27.5}&\bestcell{40.0}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Agg)*}&
\bestcell{\textcolor{blue}{37.6}}&\bestcell{\textcolor{blue}{39.7}}&\bestcell{35.8}&\bestcell{\textcolor{blue}{38.0}}&\bestcell{\textcolor{blue}{41.7}}&\bestcell{\textcolor{blue}{48.7}}&\bestcell{\textcolor{blue}{39.4}}&\bestcell{\textcolor{blue}{38.2}}&\bestcell{\textcolor{blue}{50.3}}&\bestcell{\textcolor{blue}{53.3}}&\bestcell{\textcolor{blue}{41.4}}&\bestcell{\textcolor{blue}{39.4}}&\bestcell{\textcolor{blue}{39.7}}&\bestcell{\textcolor{blue}{27.4}}&\bestcell{\textcolor{blue}{27.3}}&\bestcell{\textcolor{blue}{39.9}}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Agg)*}&
\bestcell{\textcolor{red}{37.3}}&\bestcell{\textcolor{red}{39.5}}&\bestcell{\textcolor{red}{35.6}}&\bestcell{\textcolor{red}{37.8}}&\bestcell{\textcolor{red}{41.3}}&\bestcell{\textcolor{red}{48.2}}&\bestcell{\textcolor{red}{39.1}}&\bestcell{\textcolor{red}{37.6}}&\bestcell{\textcolor{red}{49.9}}&\bestcell{\textcolor{red}{52.8}}&\bestcell{\textcolor{red}{41.2}}&\bestcell{\textcolor{red}{39.2}}&\bestcell{\textcolor{red}{39.4}}&\bestcell{\textcolor{red}{27.2}}&\bestcell{\textcolor{red}{27.1}}&\bestcell{\textcolor{red}{39.5}}
\\

\noalign{\smallskip}
\hline
\noalign{\smallskip}

MDN~\cite{li2019generating} CVPR'19 ($N$=1, $H$=5, P-Best$\sharp$)&
43.8&48.6&49.1&49.8&57.6&64.5&45.9&48.3&62.0&73.4&54.8&50.6&56.0&43.4&45.5&52.7\\
CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Best$\sharp$)&
37.8&43.2&43.0&44.3&51.1&57.0&39.7&43.0&56.3&64.0&48.1&45.4&50.4&37.9&39.9&46.8\\
GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Best$\sharp$)&
62.0&69.7&64.3&73.6&75.1&84.8&68.7&75.0&81.2&104.3&70.2&72.0&75.0&67.0&69.0&73.9\\
GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=200, P-Best$\sharp$)&
40.0&43.2&41.0&43.4&50.0&53.6&40.1&41.4&52.6&67.3&48.1&44.2&49.0&39.5&40.2&46.2\\
NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=200, P-Best$\sharp$)&
38.5&42.5&39.9&41.7&46.5&51.6&39.9&40.8&\textcolor{blue}{49.5}&56.8&45.3&46.4&46.8&37.8&40.4&44.3\\

\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Best$\sharp$)*}&
\bestcell{37.7}&\bestcell{39.9}&\bestcell{35.7}&\bestcell{38.2}&\bestcell{41.9}&\bestcell{48.8}&\bestcell{39.5}&\bestcell{38.3}&\bestcell{50.5}&\bestcell{53.9}&\bestcell{41.6}&\bestcell{39.4}&\bestcell{39.8}&\bestcell{27.4}&\bestcell{27.5}&\bestcell{40.0}
\\

\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Best$\sharp$)*}&
\bestcell{\textcolor{blue}{37.3}}&\bestcell{\textcolor{blue}{39.4}}&\bestcell{\textcolor{blue}{35.4}}&\bestcell{\textcolor{blue}{37.8}}&\bestcell{\textcolor{blue}{41.3}}&\bestcell{\textcolor{blue}{48.1}}&\bestcell{\textcolor{blue}{39.0}}&\bestcell{\textcolor{blue}{37.9}}&\bestcell{49.8}&\bestcell{\textcolor{blue}{52.8}}&\bestcell{\textcolor{blue}{41.1}}&\bestcell{\textcolor{blue}{39.0}}&\bestcell{\textcolor{blue}{39.4}}&\bestcell{\textcolor{blue}{27.3}}&\bestcell{\textcolor{blue}{27.2}}&\bestcell{\textcolor{blue}{39.5}}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Best$\sharp$)*}&
\bestcell{\textcolor{red}{33.0}}&\bestcell{\textcolor{red}{34.8}}&\bestcell{\textcolor{red}{31.7}}&\bestcell{\textcolor{red}{33.1}}&\bestcell{\textcolor{red}{37.5}}&\bestcell{\textcolor{red}{43.7}}&\bestcell{\textcolor{red}{34.8}}&\bestcell{\textcolor{red}{33.6}}&\bestcell{\textcolor{red}{45.7}}&\bestcell{\textcolor{red}{47.8}}&\bestcell{\textcolor{red}{37.0}}&\bestcell{\textcolor{red}{35.0}}&\bestcell{\textcolor{red}{35.0}}&\bestcell{\textcolor{red}{24.3}}&\bestcell{\textcolor{red}{24.1}}&\bestcell{\textcolor{red}{35.4}}
\\
\noalign{\smallskip}

\hline
\end{tabular}}
\end{center}

==> table/h36m_gt.tex <==
\begin{center}
  %\centering
  %\renewcommand\tabcolsep{4.0pt}
%\vspace{-0.5cm}
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccccccccccccccc|c}
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Deterministic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
TCN~\cite{pavllo20193d} CVPR'19 ($N$=243)& 35.2&40.2&32.7&35.7&38.2&45.5&40.6&36.1&48.8&47.3&37.8&39.7&38.7&27.8&29.5&37.8 \\
% Lin \textit{et al.}~\cite{lin2019trajectory} BMVC'19 ($N$=50)& 42.5&44.8&42.6&44.2&48.5&57.1&42.6&41.4&56.5&64.5&47.4&43.0&48.1&33.0&35.1&46.6 \\
% Xu \textit{et al.}~\cite{xu2020deep} CVPR'20 ($N$=9)
% &\textbf{37.4}&43.5&42.7&42.7&46.6&59.7&41.3&45.1&\textbf{52.7}&60.2&45.8&43.1&47.7&33.7&37.1&45.6\\
% Wang \textit{et al.}~\cite{wang2020motion} ECCV'20 ($N$=96)
% &41.3&43.9&44.0&42.2&48.0&57.1&42.2&43.2&57.3&61.3&47.0&43.5&47.0&32.6&31.8&45.6\\
% Attn-TCN~\cite{liu2020attention} CVPR'20 ($N$=243)& 41.8&44.8&41.1&44.9&47.4&54.1&43.4&42.2&56.2&63.6&45.3&43.5&45.3&31.3&32.2&45.1 \\
SRNet~\cite{zeng2020srnet} ECCV'20 ($N$=243)& 34.8&32.1&28.5&30.7&31.4&36.9&35.6&30.5&38.9&40.5&32.5&31.0&29.9&22.5&24.5&32.0 \\
% Zeng \textit{et al.}~\cite{zeng2021learning} ICCV'21 ($N$=9)
% &-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&45.7\\
Anatomy~\cite{chen2021anatomy} TCSVT'21 ($N$=243)&
-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&32.3\\
PoseFormer~\cite{zheng20213d} ICCV'21 ($N$=81)&
30.0&33.6&29.9&31.0&30.2&33.3&34.8&31.4&37.8&38.6&31.7&31.5&29.0&23.3&23.1&31.3\\
RIE~\cite{shan2021improving} ACMMM'21 ($N$=243)&
29.5&30.8&28.8&29.1&30.7&35.2&31.7&27.8&34.5&36.0&30.3&29.4&28.9&24.1&24.7&30.1\\
% U-CDGCN~\cite{hu2021conditional} ACMMM'21 ($N$=96)*&
% 38.0&43.3&39.1&\textcolor{blue}{39.4}&45.8&53.6&41.4&41.4&55.5&61.9&44.6&41.9&44.5&31.6&29.4&43.4\\
Ray3D~\cite{zhan2022ray3d} CVPR'22 ($N=9$)&
31.2&35.7&34.6&33.6&35.0&37.5&37.2&30.9&42.5&41.3&34.6&36.5&32.0&29.7&28.9&34.4\\
P-STMO~\cite{shan2022p} ECCV'22 ($N$=243)&
28.5&30.1&28.6&27.9&29.8&33.2&31.3&27.8&36.0&37.4&29.7&29.5&28.1&21.0&21.0&29.3\\
STE~\cite{li2022exploiting} TMM'22 ($N$=351)&
27.1&29.4&26.5&27.1&28.6&33.0&30.7&26.8&38.2&34.7&29.1&29.8&26.8&19.1&19.8&28.5\\
DUE~\cite{zhang2022uncertainty} ACMMM'22 ($N$=300)&
22.1&23.1&\textcolor{blue}{20.1}&22.7&21.3&24.1&\textcolor{blue}{23.6}&\textcolor{blue}{21.6}&26.3&24.8&21.7&21.4&21.8&16.7&18.7&22.0\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)&
\textcolor{blue}{21.6}&22.0&20.4&\textcolor{blue}{21.0}&\textcolor{blue}{20.8}&26.3&24.7&21.9&26.9&24.9&\textcolor{blue}{21.2}&21.5&20.8&\textcolor{blue}{14.7}&\textcolor{blue}{15.7}&21.6\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)$\ddagger$&
22.9&\textcolor{blue}{21.7}&21.0&21.4&\textcolor{blue}{20.8}&\textcolor{blue}{23.5}&24.1&21.8&\textcolor{red}{25.3}&\textcolor{red}{23.5}&21.4&\textcolor{blue}{20.1}&\textcolor{blue}{19.5}&15.3&16.6&\textcolor{blue}{21.3}\\

\bestcell{D3DP ($N$=243, $H$=1, $K$=1)}&
\bestcell{\textcolor{red}{19.9}}&\bestcell{\textcolor{red}{19.6}}&\bestcell{\textcolor{red}{19.7}}&\bestcell{\textcolor{red}{19.3}}&\bestcell{\textcolor{red}{20.2}}&\bestcell{\textcolor{red}{22.7}}&\bestcell{\textcolor{red}{21.5}}&\bestcell{\textcolor{red}{19.2}}&\bestcell{\textcolor{blue}{25.5}}&\bestcell{\textcolor{blue}{24.0}}&\bestcell{\textcolor{red}{20.1}}&\bestcell{\textcolor{red}{18.9}}&\bestcell{\textcolor{red}{19.0}}&\bestcell{\textcolor{red}{14.0}}&\bestcell{\textcolor{red}{14.5}}&\bestcell{\textcolor{red}{19.9}}\\
\noalign{\smallskip}
\hline
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Probabilistic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
% MDN~\cite{li2019generating} CVPR'19 ($N$=1, $H$=5, P-Best$\sharp$)$\ddagger$&
% 43.8&48.6&49.1&49.8&57.6&64.5&45.9&48.3&62.0&73.4&54.8&50.6&56.0&43.4&45.5&52.7\\
% CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Agg)$\ddagger$&
% 48.6&54.5&54.2&55.7&62.6&72.0&50.5&54.3&70.0&78.3&58.1&55.4&61.4&45.2&49.7&58.0\\
% CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Best$\sharp$)$\ddagger$&
% 37.8&43.2&43.0&44.3&51.1&57.0&39.7&43.0&56.3&64.0&48.1&45.4&50.4&37.9&39.9&46.8\\
% GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Agg)$\ddagger$&
% 67.9&75.5&71.8&81.8&81.4&93.7&75.2&81.3&88.8&114.1&75.9&79.1&83.3&74.3&79.0&81.1\\

GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=5, P-Agg)&
33.9&39.9&33.0&35.4&36.8&44.4&38.9&33.0&41.0&50.0&36.4&38.3&37.8&28.2&31.5&37.2\\
MHFormer~\cite{li2022mhformer} CVPR'22 ($N$=351, $H$=3, P-Agg)&
\textcolor{blue}{27.7}&32.1&29.1&28.9&30.0&33.9&33.0&31.2&37.0&39.3&30.3&31.0&29.4&\textcolor{blue}{22.2}&\textcolor{blue}{23.0}&30.5
\\
\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Agg)}&
\bestcell{\textcolor{red}{19.9}}&\bestcell{19.6}&\bestcell{19.7}&\bestcell{19.3}&\bestcell{20.2}&\bestcell{22.7}&\bestcell{\textcolor{blue}{21.5}}&\bestcell{\textcolor{blue}{19.2}}&\bestcell{25.5}&\bestcell{24.0}&\bestcell{20.1}&\bestcell{\textcolor{blue}{18.9}}&\bestcell{19.0}&\bestcell{\textcolor{red}{14.0}}&\bestcell{\textcolor{red}{14.5}}&\bestcell{19.9}\\

\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Agg)}&
\bestcell{\textcolor{red}{19.9}}&\bestcell{\textcolor{blue}{19.5}}&\bestcell{\textcolor{blue}{19.6}}&\bestcell{\textcolor{blue}{19.2}}&\bestcell{\textcolor{blue}{20.1}}&\bestcell{\textcolor{blue}{22.4}}&\bestcell{\textcolor{blue}{21.5}}&\bestcell{\textcolor{red}{19.1}}&\bestcell{\textcolor{blue}{25.4}}&\bestcell{\textcolor{blue}{23.7}}&\bestcell{\textcolor{blue}{20.0}}&\bestcell{\textcolor{blue}{18.9}}&\bestcell{\textcolor{blue}{18.8}}&\bestcell{\textcolor{red}{14.0}}&\bestcell{\textcolor{red}{14.5}}&\bestcell{\textcolor{blue}{19.8}}\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Agg)}&
\bestcell{\textcolor{red}{19.9}}&\bestcell{\textcolor{red}{19.4}}&\bestcell{\textcolor{red}{19.4}}&\bestcell{\textcolor{red}{19.0}}&\bestcell{\textcolor{red}{19.8}}&\bestcell{\textcolor{red}{22.0}}&\bestcell{\textcolor{red}{21.4}}&\bestcell{\textcolor{red}{19.1}}&\bestcell{\textcolor{red}{24.8}}&\bestcell{\textcolor{red}{23.2}}&\bestcell{\textcolor{red}{19.6}}&\bestcell{\textcolor{red}{18.7}}&\bestcell{\textcolor{red}{18.6}}&\bestcell{\textcolor{red}{14.0}}&\bestcell{\textcolor{red}{14.5}}&\bestcell{\textcolor{red}{19.6}}
\\

\noalign{\smallskip}
\hline
\noalign{\smallskip}


GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Best$\sharp$)&
54.8&61.9&48.6&63.6&55.8&73.7&59.0&61.3&62.2&85.7&52.8&60.2&57.5&51.3&56.8&60.0\\
GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=5, P-Best$\sharp$)&
28.9&34.5&28.2&30.2&31.5&38.5&32.3&28.6&35.7&43.3&31.9&32.1&33.3&25.2&27.8&31.8\\
% NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=1)$\vartriangle$&
% 52.4&60.2&57.8&57.4&65.7&74.1&56.2&59.1&69.3&78.0&61.2&63.7&67.0&50.0&54.9&61.8\\
% NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=200, P-Best$\sharp$)$\vartriangle$&
% 38.5&42.5&39.9&41.7&46.5&51.6&39.9&40.8&49.5&56.8&45.3&46.4&46.8&37.8&40.4&44.3\\

\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Best$\sharp$)}&
\bestcell{19.9}&\bestcell{19.6}&\bestcell{19.7}&\bestcell{19.3}&\bestcell{20.2}&\bestcell{22.7}&\bestcell{21.5}&\bestcell{19.2}&\bestcell{25.5}&\bestcell{24.0}&\bestcell{20.1}&\bestcell{18.9}&\bestcell{19.0}&\bestcell{14.0}&\bestcell{14.5}&\bestcell{19.9}\\

\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Best$\sharp$)}&
\bestcell{\textcolor{blue}{19.7}}&\bestcell{\textcolor{blue}{19.3}}&\bestcell{\textcolor{blue}{19.2}}&\bestcell{\textcolor{blue}{18.8}}&\bestcell{\textcolor{blue}{19.6}}&\bestcell{\textcolor{blue}{21.9}}&\bestcell{\textcolor{blue}{21.2}}&\bestcell{\textcolor{blue}{18.6}}&\bestcell{\textcolor{blue}{24.7}}&\bestcell{\textcolor{blue}{23.0}}&\bestcell{\textcolor{blue}{19.4}}&\bestcell{\textcolor{blue}{18.4}}&\bestcell{\textcolor{blue}{18.4}}&\bestcell{\textcolor{blue}{13.9}}&\bestcell{\textcolor{blue}{14.4}}&\bestcell{\textcolor{blue}{19.4}}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Best$\sharp$)}&
\bestcell{\textcolor{red}{18.7}}&\bestcell{\textcolor{red}{18.2}}&\bestcell{\textcolor{red}{18.4}}&\bestcell{\textcolor{red}{17.8}}&\bestcell{\textcolor{red}{18.6}}&\bestcell{\textcolor{red}{20.9}}&\bestcell{\textcolor{red}{20.2}}&\bestcell{\textcolor{red}{17.7}}&\bestcell{\textcolor{red}{23.8}}&\bestcell{\textcolor{red}{21.8}}&\bestcell{\textcolor{red}{18.5}}&\bestcell{\textcolor{red}{17.4}}&\bestcell{\textcolor{red}{17.4}}&\bestcell{\textcolor{red}{13.1}}&\bestcell{\textcolor{red}{13.6}}&\bestcell{\textcolor{red}{18.4}}
\\
\noalign{\smallskip}

\hline
\end{tabular}}
\end{center}

==> table/h36m_pmpjpe.tex <==
\begin{center}
  %\centering
  %\renewcommand\tabcolsep{4.0pt}
%\vspace{-0.5cm}
\resizebox{\textwidth}{!}{\begin{tabular}{c|ccccccccccccccc|c}
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Deterministic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
P-MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
TCN~\cite{pavllo20193d} CVPR'19 ($N$=243)*& 34.1&36.1&34.4&37.2&36.4&42.2&34.4&33.6&45.0&52.5&37.4&33.8&37.8&25.6&27.3&36.5 \\
% Lin \textit{et al.}~\cite{lin2019trajectory} BMVC'19 ($N$=50)& 42.5&44.8&42.6&44.2&48.5&57.1&42.6&41.4&56.5&64.5&47.4&43.0&48.1&33.0&35.1&46.6 \\
% Xu \textit{et al.}~\cite{xu2020deep} CVPR'20 ($N$=9)
% &\textbf{37.4}&43.5&42.7&42.7&46.6&59.7&41.3&45.1&\textbf{52.7}&60.2&45.8&43.1&47.7&33.7&37.1&45.6\\
% Wang \textit{et al.}~\cite{wang2020motion} ECCV'20 ($N$=96)
% &41.3&43.9&44.0&42.2&48.0&57.1&42.2&43.2&57.3&61.3&47.0&43.5&47.0&32.6&31.8&45.6\\
% Attn-TCN~\cite{liu2020attention} CVPR'20 ($N$=243)& 41.8&44.8&41.1&44.9&47.4&54.1&43.4&42.2&56.2&63.6&45.3&43.5&45.3&31.3&32.2&45.1 \\
% SRNet~\cite{zeng2020srnet} ECCV'20 ($N$=243)*& 46.6&47.1&43.9&41.6&45.8&49.6&46.5&40.0&53.4&61.1&46.1&42.6&43.1&31.5&32.6&44.8 \\
% Zeng \textit{et al.}~\cite{zeng2021learning} ICCV'21 ($N$=9)
% &-&-&-&-&-&-&-&-&-&-&-&-&-&-&-&45.7\\
RIE~\cite{shan2021improving} ACMMM'21 ($N$=243)*&
32.5&36.2&33.2&35.3&35.6&42.1&32.6&31.9&42.6&47.9&36.6&32.1&34.8&24.2&25.8&35.0\\
Anatomy~\cite{chen2021anatomy} TCSVT'21 ($N$=243)*&
32.6&35.1&32.8&35.4&36.3&40.4&32.4&32.3&42.7&49.0&36.8&32.4&36.0&24.9&26.5&35.0\\
PoseFormer~\cite{zheng20213d} ICCV'21 ($N$=81)*&
32.5&34.8&32.6&34.6&35.3&39.5&32.1&32.0&42.8&48.5&34.8&32.4&35.3&24.5&36.0&34.6\\
U-CDGCN~\cite{hu2021conditional} ACMMM'21 ($N$=96)*&
\textcolor{red}{29.8}&34.4&31.9&\textcolor{blue}{31.5}&35.1&40.0&\textcolor{red}{30.3}&30.8&42.6&49.0&35.9&31.8&35.0&25.7&23.6&33.8\\
% Ray3D~\cite{zhan2022ray3d} CVPR'22 ($N=9$)*&
% 44.7&48.7&48.7&48.4&51.0&59.9&46.8&46.9&58.7&61.7&50.2&46.4&51.5&38.6&41.8&49.7\\
STE~\cite{li2022exploiting} TMM'22 ($N$=351)*&
32.7&35.5&32.5&35.4&35.9&41.6&33.0&31.9&45.1&50.1&36.3&33.5&35.1&23.9&25.0&35.2\\
P-STMO~\cite{shan2022p} ECCV'22 ($N$=243)*&
31.3&35.2&32.9&33.9&35.4&39.3&32.5&31.5&44.6&48.2&36.3&32.9&34.4&23.8&23.9&34.4\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)*&
30.8&33.1&30.3&31.8&33.1&39.1&31.1&30.5&42.5&44.5&34.0&30.8&32.7&22.1&22.9&32.6\\
MixSTE~\cite{zhang2022mixste} CVPR'22 ($N$=243)*$\ddagger$&
30.8&\textcolor{blue}{32.7}&30.6&31.9&33.1&\textcolor{blue}{38.6}&\textcolor{blue}{30.8}&\textcolor{blue}{30.4}&42.4&46.4&34.2&\textcolor{blue}{30.7}&\textcolor{blue}{32.3}&\textcolor{blue}{21.8}&\textcolor{blue}{22.6}&32.6\\
DUE~\cite{zhang2022uncertainty} ACMMM'22 ($N$=300)*&
\textcolor{blue}{30.3}&34.6&\textcolor{blue}{29.6}&31.7&\textcolor{red}{31.6}&38.9&31.8&31.9&\textcolor{red}{39.2}&\textcolor{red}{42.8}&\textcolor{red}{32.1}&32.6&\textcolor{red}{31.4}&25.1&23.8&\textcolor{blue}{32.5}\\

\bestcell{D3DP ($N$=243, $H$=1, $K$=1)*}&
\bestcell{30.6}&\bestcell{\textcolor{red}{32.5}}&\bestcell{\textcolor{red}{29.1}}&\bestcell{\textcolor{red}{31.0}}&\bestcell{\textcolor{blue}{31.9}}&\bestcell{\textcolor{red}{37.6}}&\bestcell{\textcolor{red}{30.3}}&\bestcell{\textcolor{red}{29.4}}&\bestcell{\textcolor{blue}{40.6}}&\bestcell{\textcolor{blue}{43.6}}&\bestcell{\textcolor{blue}{33.3}}&\bestcell{\textcolor{red}{30.5}}&\bestcell{\textcolor{red}{31.4}}&\bestcell{\textcolor{red}{21.5}}&\bestcell{\textcolor{red}{22.4}}&\bestcell{\textcolor{red}{31.7}}\\

\noalign{\smallskip}
\hline
\hline
\noalign{\smallskip}
%\rowcolor[HTML]{DADADA}
\multicolumn{17}{c}{\textbf{\large{Probabilistic Methods}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
P-MPJPE & Dir. & Disc. & Eat & Greet & Phone & Photo & Pose & Pur. & Sit & SitD. & Smoke & Wait & WalkD. & Walk & WalkT. & Avg \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}

CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Agg)&
35.3&35.9&45.8&42.0&40.9&52.6&36.9&35.8&43.5&51.9&44.3&38.8&45.5&29.4&34.3&40.9\\
GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Agg)&
42.1&44.7&45.4&51.0&49.3&51.5&41.2&46.2&57.5&70.8&48.7&44.1&50.8&42.1&43.7&48.7\\
GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=5, P-Agg)&
39.7&43.4&44.0&46.2&48.8&54.5&39.4&41.1&55.0&69.0&48.0&43.7&49.6&38.4&42.4&46.9\\
NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=1, P-Agg)&
37.8&41.7&42.1&41.8&46.5&50.2&38.0&39.2&51.7&61.8&45.4&42.6&45.7&33.7&38.5&43.8\\
MHFormer~\cite{li2022mhformer} CVPR'22 ($N$=351, $H$=3, P-Agg)*&
\textcolor{blue}{31.5}&34.9&32.8&33.6&\textcolor{blue}{35.3}&39.6&32.0&32.2&43.5&48.7&36.4&32.6&34.3&\textcolor{blue}{23.9}&25.1&34.4
\\
\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Agg)*}&
\bestcell{\textcolor{red}{30.6}}&\bestcell{\textcolor{blue}{32.5}}&\bestcell{\textcolor{red}{29.1}}&\bestcell{\textcolor{blue}{31.0}}&\bestcell{\textcolor{red}{31.9}}&\bestcell{37.6}&\bestcell{\textcolor{blue}{30.3}}&\bestcell{\textcolor{blue}{29.4}}&\bestcell{\textcolor{blue}{40.6}}&\bestcell{43.6}&\bestcell{\textcolor{blue}{33.3}}&\bestcell{\textcolor{blue}{30.5}}&\bestcell{\textcolor{blue}{31.4}}&\bestcell{\textcolor{red}{21.5}}&\bestcell{\textcolor{blue}{22.4}}&\bestcell{\textcolor{blue}{31.7}}\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Agg)*}&
\bestcell{\textcolor{red}{30.6}}&\bestcell{\textcolor{blue}{32.5}}&\bestcell{\textcolor{red}{29.1}}&\bestcell{\textcolor{red}{30.9}}&\bestcell{\textcolor{red}{31.9}}&\bestcell{\textcolor{blue}{37.5}}&\bestcell{\textcolor{red}{30.2}}&\bestcell{\textcolor{blue}{29.4}}&\bestcell{\textcolor{blue}{40.6}}&\bestcell{\textcolor{blue}{43.4}}&\bestcell{\textcolor{blue}{33.3}}&\bestcell{\textcolor{red}{30.4}}&\bestcell{\textcolor{blue}{31.4}}&\bestcell{\textcolor{red}{21.5}}&\bestcell{\textcolor{blue}{22.4}}&\bestcell{\textcolor{blue}{31.7}}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Agg)*}&
\bestcell{\textcolor{red}{30.6}}&\bestcell{\textcolor{red}{32.4}}&\bestcell{\textcolor{blue}{29.2}}&\bestcell{\textcolor{red}{30.9}}&\bestcell{\textcolor{red}{31.9}}&\bestcell{\textcolor{red}{37.4}}&\bestcell{\textcolor{red}{30.2}}&\bestcell{\textcolor{red}{29.3}}&\bestcell{\textcolor{red}{40.4}}&\bestcell{\textcolor{red}{43.2}}&\bestcell{\textcolor{red}{33.2}}&\bestcell{\textcolor{red}{30.4}}&\bestcell{\textcolor{red}{31.3}}&\bestcell{\textcolor{red}{21.5}}&\bestcell{\textcolor{red}{22.3}}&\bestcell{\textcolor{red}{31.6}}
\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}


MDN~\cite{li2019generating} CVPR'19 ($N$=1, $H$=5, P-Best$\sharp$)&
35.5&39.8&41.3&42.3&46.0&48.9&36.9&37.3&51.0&60.6&44.9&40.2&44.1&33.1&36.9&42.6\\
CVAE~\cite{sharma2019monocular} ICCV'19 ($N$=1, $H$=200, P-Best$\sharp$)&
\textcolor{blue}{27.6}&\textcolor{red}{27.5}&34.9&32.3&33.3&42.7&28.7&\textcolor{blue}{28.0}&\textcolor{red}{36.1}&42.7&36.0&30.7&37.6&24.3&27.1&32.7\\
GAN~\cite{li2020weakly} BMVC'20 ($N$=1, $H$=10, P-Best$\sharp$)&
38.5&41.7&39.6&45.2&45.8&46.5&37.8&42.7&52.4&62.9&45.3&40.9&45.3&38.6&38.4&44.3\\
GraphMDN~\cite{oikarinen2021graphmdn} IJCNN'21 ($N$=1, $H$=200, P-Best$\sharp$)&
30.8&34.7&33.6&34.2&39.6&42.2&31.0&31.9&42.9&53.5&38.1&34.1&38.0&29.6&31.1&36.3\\
NF~\cite{wehrbein2021probabilistic} ICCV'21 ($N$=1, $H$=200, P-Best$\sharp$)&
27.9&31.4&29.7&\textcolor{blue}{30.2}&34.9&37.1&\textcolor{red}{27.3}&28.2&39.0&46.1&34.2&32.3&33.6&26.1&27.5&32.4\\

\bestcell{D3DP ($N$=243, $H$=1, $K$=1, P-Best$\sharp$)*}&
\bestcell{30.6}&\bestcell{32.5}&\bestcell{29.1}&\bestcell{31.0}&\bestcell{31.9}&\bestcell{37.6}&\bestcell{30.3}&\bestcell{29.4}&\bestcell{40.6}&\bestcell{43.6}&\bestcell{33.3}&\bestcell{30.5}&\bestcell{31.4}&\bestcell{21.5}&\bestcell{22.4}&\bestcell{31.7}\\

\bestcell{D3DP ($N$=243, $H$=20, $K$=10, P-Best$\sharp$)*}&
\bestcell{30.2}&\bestcell{32.1}&\bestcell{\textcolor{blue}{28.8}}&\bestcell{30.4}&\bestcell{\textcolor{blue}{31.5}}&\bestcell{\textcolor{blue}{37.0}}&\bestcell{29.8}&\bestcell{28.9}&\bestcell{39.9}&\bestcell{\textcolor{blue}{42.4}}&\bestcell{\textcolor{blue}{32.8}}&\bestcell{\textcolor{blue}{30.0}}&\bestcell{\textcolor{blue}{30.9}}&\bestcell{\textcolor{blue}{21.3}}&\bestcell{\textcolor{blue}{22.1}}&\bestcell{\textcolor{blue}{31.2}}
\\
\bestcell{D3DP ($N$=243, $H$=20, $K$=10, J-Best$\sharp$)*}&
\bestcell{\textcolor{red}{27.5}}&\bestcell{\textcolor{blue}{29.4}}&\bestcell{\textcolor{red}{26.6}}&\bestcell{\textcolor{red}{27.7}}&\bestcell{\textcolor{red}{29.2}}&\bestcell{\textcolor{red}{34.3}}&\bestcell{\textcolor{blue}{27.5}}&\bestcell{\textcolor{red}{26.2}}&\bestcell{\textcolor{blue}{37.3}}&\bestcell{\textcolor{red}{39.0}}&\bestcell{\textcolor{red}{30.3}}&\bestcell{\textcolor{red}{27.7}}&\bestcell{\textcolor{red}{28.2}}&\bestcell{\textcolor{red}{19.6}}&\bestcell{\textcolor{red}{20.3}}&\bestcell{\textcolor{red}{28.7}}
\\
\noalign{\smallskip}

\hline
\end{tabular}}
\end{center}
